How Good are Low-Rank Approximations in Gaussian Process Regression?

We provide guarantees for approximate Gaussian Process (GP) regression resulting from two common low-rank kernel approximations: based on random Fourier features, and based on truncating the kernel's Mercer expansion. In particular, we bound the Kullback-Leibler divergence between an exact GP and one resulting from one of the afore-described low-rank approximations to its kernel, as well as between their corresponding predictive densities, and we also bound the error between predictive mean vectors and between predictive covariance matrices computed using the exact versus using the approximate GP. We provide experiments on both simulated data and standard benchmarks to evaluate the effectiveness of our theoretical bounds.

==> conclusion.tex <==
\section{Conclusion}
We have investigated, both theoretically and practically, the accuracy of low-rank approximations for GP regression based on random Fourier features and  truncating Mercer expansion. We have bounded the KL divergence between the true marginal likelihood of GP and the marginal likelihood of an approximate GP. These bounds are inextricably linked with the decay rate of kernel's eigenspectrum, implying that data concentrated in small regions in tandem with smooth kernels lead to very accurate results for approximate GP regression with small rank. Results on real-world datasets also confirms our theoretical analysis.   An interesting future direction is the derivation of similar theoretical bounds for non-Gaussian likelihoods.  A further research topic that was revealed when performing the experiments in the real data examples is to investigate our proposed feature projection to a dimension $d<D$ and the corresponding optimum choice of the first $r$ eigenfunctions of Mercer expansion for multivariate data with anisotropic behavior.  
